Wind-MRI interactions in local models of protoplanetary discs: I. Ohmic resistivity

A magnetic disc wind is an important mechanism that may be responsible for driving accretion and structure formation in protoplanetary discs. Recent numerical simulations have shown that these winds can take either the traditional `hourglass' symmetry about the mid-plane, or a `slanted' symmetry dominated by a mid-plane toroidal field of a single sign. The formation of this slanted symmetry state has not previously been explained. We use radially local 1D vertical shearing box simulations to assess the importance of large-scale MRI channel modes in influencing the formation and morphologies of these wind solutions. We consider only Ohmic resistivity and explore the effect of different magnetisations, with the mid-plane $\beta$ parameter ranging from $10^5$ to $10^2$. We find that our magnetic winds go through three stages of development: cyclic, transitive and steady, with the steady wind taking a slanted symmetry profile similar to those observed in local and global simulations. We show that the cycles are driven by periodic excitation of the $n=2$ or $3$ MRI channel mode coupled with advective eviction, and that the transition to the steady wind is caused by a much more slowly growing $n=1$ mode altering the wind structure. Saturation is achieved through a combination of advective damping from the strong wind, and suppression of the instability due to a strong toroidal field. A higher disc magnetisation leads to a greater tendency towards, and more rapid settling into the slanted symmetry steady wind, which may have important implications for mass and flux transport processes in protoplanetary discs.

==> Introduction.tex <==
\section{Introduction}

This is a simple template for authors to write new MNRAS papers.
See \texttt{mnras\_sample.tex} for a more complex example, and \texttt{mnras\_guide.tex}
for a full user guide.

All papers should start with an Introduction section, which sets the work
in context, cites relevant earlier studies in the field by \citet{Others2013},
and describes the problem the authors aim to solve \citep[e.g.][]{Author2012}.

==> NotUsedText.tex <==
[In PPDs, we can assume that the recombination time is much shorter than the dynamical time ($\Omega^{-1}$)  \citep{Bai2011a}. Hence we are in the strong coupling limit \citep{Shu_1991} where local ionisation equilibrium is a good approximation of disc microphysics. This allows us to compute magnetic diffusivities from local thermodynamic quantities such as density and temperature and the ionisation rate.]

[\citet{BaiStone2011} performed 3D unstratified shearing box in the ambipolar diffusion regime. They found that the MRI is suppressed when the field strength exceeds a threshold value (when $\langle \beta\rangle \leq \beta_\text{min}(\Lambda_A)$). They also confirmed the results of analytic studies that in the weak field limit, MRI turbulence is generated regardless of the ambipolar strength, although its magnitude also decreases rapidly as $\Lambda_A$ drops below unity. It is worth noting that analytic investigations on the linear growth of the MRI with both Hall drift and ambipolar diffusion were done by \citep{SalmeronWardle_2003,SalmeronWardle_2005} for a stratified disc. They predicted that in this regime, global modes are possible in the disc even in the strong field (low $\beta$) regime and with a small $\Lambda_A$. This result is yet to be verified in stratified shearing box simulations.]

We also identified that the flux transport due to the `Hydro' and $D_B$ source terms share the same qualitative trends in its variation with Ohmic resistivity, while for Hall diffusivity they also share the same trend as the $b_{rs}$ source term. 
